Neural Volume Super-Resolution

Neural volumetric representations have become a widely adopted model for radiance fields in 3D scenes. These representations are fully implicit or hybrid function approximators of the instantaneous volumetric radiance in a scene, which are typically learned from multi-view captures of the scene. We investigate the new task of neural volume super-resolution - rendering high-resolution views corresponding to a scene captured at low resolution. To this end, we propose a neural super-resolution network that operates directly on the volumetric representation of the scene. This approach allows us to exploit an advantage of operating in the volumetric domain, namely the ability to guarantee consistent super-resolution across different viewing directions. To realize our method, we devise a novel 3D representation that hinges on multiple 2D feature planes. This allows us to super-resolve the 3D scene representation by applying 2D convolutional networks on the 2D feature planes. We validate the proposed method by super-resolving multi-view consistent views on a diverse set of unseen 3D scenes, confirming qualitative and quantitatively favorable quality over existing approaches.

==> figures/real_results.tex <==
\begin{figure*}[!htp]
\centering
\includegraphics[width=\textwidth]{images/results.pdf}
\caption{\label{fig:real_results}\textbf{\yb{Placeholder images}Super-resolution of real scenes.}
We visually compare the performance of our method (right) to performance by leading SR methods and baselines, when super resolving novel low-resolution views (left). Our Neural Volume SR approach is able to reconstruct finer details and smaller structures compared to all other methods. While operating naively in the volumetric domain by interpolating the feature planes (2\textsuperscript{nd} from right) already yields visual benefit, applying our SR model $F$ on the planes achieves a significant improvement.
}
\end{figure*}


==> tables/zero_mean_penalty.tex <==
\begin{table}[!ht]
    \centering
    \begin{tabular}{ccccc}
        \toprule
        ${\cal L}_P$ & PSNR $(db)(\uparrow)$&SSIM $(\uparrow)$& LPIPS $(\downarrow)$\\
        \midrule 
        With&  $\textbf{25.682}$ &$0.823$ & $0.264$\\
        Without& $25.655$ & $0.823$ & $\textbf{0.259}$\\
        \bottomrule
    \end{tabular}
    % }
    \caption{\textbf{Effect of penalty ${\cal L}_P$ over per-feature spatial mean.}
    We compare reconstruction performance of our framework trained with vs. without penalty term ${\cal L}_P$ which encourages a per-feature zero mean for our model's feature planes. For each experiment and metric we also measure performance without super-resolving the feature planes and report them in parentheses.
    }
    \label{tab:zero_mean_penalty}
\end{table}
